Loss Function Discovery for Object Detection via Convergence-Simulation Driven Search

Designing proper loss functions for vision tasks has been a long-standing research direction to advance the capability of existing models. For object detection, the well-established classification and regression loss functions have been carefully designed by considering diverse learning challenges. Inspired by the recent progress in network architecture search, it is interesting to explore the possibility of discovering new loss function formulations via directly searching the primitive operation combinations. So that the learned losses not only fit for diverse object detection challenges to alleviate huge human efforts, but also have better alignment with evaluation metric and good mathematical convergence property. Beyond the previous auto-loss works on face recognition and image classification, our work makes the first attempt to discover new loss functions for the challenging object detection from primitive operation levels. We propose an effective convergence-simulation driven evolutionary search algorithm, called CSE-Autoloss, for speeding up the search progress by regularizing the mathematical rationality of loss candidates via convergence property verification and model optimization simulation. CSE-Autoloss involves the search space that cover a wide range of the possible variants of existing losses and discovers best-searched loss function combination within a short time (around 1.5 wall-clock days). We conduct extensive evaluations of loss function search on popular detectors and validate the good generalization capability of searched losses across diverse architectures and datasets. Our experiments show that the best-discovered loss function combinations outperform default combinations by 1.1% and 0.8% in terms of mAP for two-stage and one-stage detectors on COCO respectively. Our searched losses are available at https://github.com/PerdonLiu/CSE-Autoloss.

==> rebuttal.tex <==
\section{Rebuttal}
\subsection{Review1}
Q: The proposed method is heavily based on the works of auto loss for image classification, i.e. "Improved Training Speed, Accuracy, and Data Utilization Through Loss Function Optimization".

A: The work "Improved Training Speed, Accuracy, and Data Utilization Through Loss Function Optimization"[1] propose a loss function search framework for image classification, which we have cited in the "RELATED WORK" part of our paper. The key difference are as follows:

- Search space. The search space of the [1] includes 3 unary operators, 4 binary operators and several inputs, while ours consist of 20 mathematical operators, which has a larger and hence more flexible search space. In addition, we further introduce IoU into classification branch search space to align with the evaluation metric for object detection, which is not mentioned in [1].
- Search algorithm. [1] apply vanilla evolutionary algorithm, while as you have pointed out, our proposed method CSE-Autoloss accelerate the search process by 20x via convergence-simulation modules. In fact, the vanilla evolutionary algorithm can meet the need for searching in small dataset like MNIST, CIFAR10 but it is not a good choice for large-scale dataset, e.g. COCO, especially for a more complex object detection task. In Table 5 of our paper, we demonstrate that vanilla evolutionary search requires 500 wall-clock hours while our proposed method only needs 34 wall-clock hours to get the best-discovered loss for both classification and regression branch, which indicates the efficiency of our proposed method.

Q: **How the method balances between classification and localization losses? Independently searching either cls or localization loss does not guarantee a good performance when combining them together for a high AP.**

A: In this work, we do search independently for classification and regression branch, with another branch fixed when searching for one branch. The evaluation experiment shows that this search mechanism can find some loss combinations outperform traditional combination by a margin. Actually, searching for classification and localization branch jointly may be a better method. We will carefully consider your constructive suggestions and validate them in our future work.

Q: **The searched loss formulation seems complex and tricky, thus raising the doubt of its generalization across a wide range of neural networks and datasets**. **Do we need to re-search the loss function once we change the network architecture or the training data slightly?**

A: There is no need to re-search the loss function when we change network slightly or use different training data. The searched loss formulations can generalize to different architectures and various datasets. In Table 3, the searched loss obtains 0.9\% and 0.8\% increase in PASCAL VOC and BDD, respectively. In Table 1, the loss searched in Faster R-CNN with ResNet50 can generalize to bigger backbone like Faster R-CNN with ResNet101, different detectors like Cascade R-CNN and Mask R-CNN. In addition, the loss searched in FCOS can also generalize well to ATSS.

\subsection{Review2}
Q: **Some related works on improving Focal loss and GIoU [1][2] are missing, it is better to include them as parts of hand-crafted loss functions for comparisons.**

A: Thanks for your kind remain. We will include CIoU/DIoU[1] and \textcolor{red}{GHM[2]} in our revised version.

Q: **Is it possible to search classification and regression loss together? It seems for now classification and regression loss are searched independently.**

A: Yes, it is possible to search two branches together. We will seriously consider your productive suggestions and accomplish it in our future work.

Q: I**t seems $Autoloss-A_cls$ and $Autoloss-B_cls$ design are quiet different. Any possible explanation for this difference?**

A: The difference between $Autoloss-A_cls$ and $Autoloss-B_cls$ is reasonable from the following two perspectives:

- The predefined initial loss for $Autoloss-A_cls$ CEI and $Autoloss-B_cls$ FLI are variants of CE loss and FL loss, respectively, which are rather different.
- The challenges for one-stage and two-stage are distinct. Specifically, one-stage suffers from severe positive-negative sample imbalance due to dense sampling of possible object locations, while two stage is free of this issue due to effective ROI pooling.


\subsection{Review3}
Q: **For the predefined initial loss, CEI/FLI loss and GIoU loss are used for classification and regression, respectively. If using other losses as the predefined initial loss, how is the performance? Could you provide some experiments?**

A: We try a different initial losses ** for regression branch and ** for classification branch in two-stage detectors. We discover a nuanced regression and classification loss: 

initial regression loss: $CSE-Autoloss-A_{reg}$
searched regression loss($search reg loss3$): Add(1,Neg(Add(Div(I,U),Neg(Div(Add(Div(E,2),Neg(U)),E)))))

initial classification loss: $CSE-Autoloss-A_{cls}$
searched classification loss ($finding1 loss1$): Neg(Dot(Mul(Y,Add(1,Z)),Log(Softmax(X))))


This experiment validates that the searched loss functions have similar performance given the same search space with different predefined initial loss.

Q: In the search experiments, regression and classification loss functions are searched independently. For me, this can not result in the optimal loss functions. Why does not search jointly?
A: 

Q: **In the evolutionary algorithm, how do the probabilities of cross-over and mutation affect the performance of searched loss?**

In our default search experiments, the probabilities of cross-over and mutation set to 0.5 and 0.2, respectively. To address your concern, we further conduct search experiments with several different probability combinations as follows:

searched regression loss(find reg 2):Add(1,Neg(Add(Div(I,U),Neg(Div(Add(E,Neg(U)),Exp(Exp(Add(Abs(E),Add(U,E)))))))))
searched regression loss(find reg 4):Add(1,Neg(Add(Div(I,U),Neg(Div(Add(E,Neg(U)),Square(Neg(Sqrt(Square(I)))))))))
searched regression loss(find reg 6):Add(1,Neg(Add(Div(I,U),Neg(Div(Add(E,Neg(U)),Sqrt(Div(Add(Exp(I),Abs(3)),Add(Abs(E),Sqrt(E)))))))))
searched regression loss(find reg 11):Add(1,Neg(Add(Div(I,U),Sqrt(Div(Exp(3),I)))))


In short, the search process is not so sensitive to the probabilities of cross-over and mutation given the well-designed search space and proper initial loss.

Q: **If directly search loss functions on these detectors and datasets, how are the performances?**

search on ATSS, searched classification loss(search cls 16): Neg(Add(Mul(Q,Mul(Add(1,Sig(Neg(Abs(Exp(X))))),Log(Sig(X)))),Mul(Add(1,Neg(Q)),Mul(Add(Add(1,Neg(Q)),Neg(Add(1,Neg(Sig(X))))),Log(Add(1,Neg(Sig(X))))))))
search on VOC, searched classification loss(find reg 9): Add(Div(U,I),Neg(Add(Div(I,U),Neg(Div(Add(E,Neg(U)),E)))))

Directly search loss functions on specific detectors and datasets can achieve small performance upgrade. The results can be found in the table below.

\subsection{Review4}
Q: **The authors should consider using baselines with better performance.** **I also wonder if the loss would generalize to different datasets, such as PASCAL VOC.**

A: Thanks for your kind remain and additional experiments are added as follows.

In our paper, we generalize the search loss to different datasets including PASCAL VOC and BDD and achieve consistent improvement in terms of mAP. The results can be found in Table 3.

Q: The authors use the modified version of the cross entropy or focal loss as the initial loss in the search experiments. The final version of the loss is still pretty much the same as the initial loss. It seems that the search is biased towards to the initial loss. I wonder if the authors have tried other initializations.

A: Yes, we have tried different initializations. In the early stage of our work, IoU is not considered in the search space. The predefined classification initial loss for two-stage detector is cross entropy loss. The searched loss is as follows:

searched classification loss(search cls loss no iou 9): Neg(Mul(Y,Log(Softmax(Add(X,Softmax(Softmax(Add(Div(Y,2),Y))))))))

Due to the lack of the alignment with the evaluation metric, this searched loss underperforms $Autoloss-A_cls$.

But if the search space is the same, the performance of the searched loss is similar.


initial regression loss: $CSE-Autoloss-A_{reg}$
searched regression loss($search reg loss3$): Add(1,Neg(Add(Div(I,U),Neg(Div(Add(Div(E,2),Neg(U)),E)))))

initial classification loss: $CSE-Autoloss-A_{cls}$
searched classification loss ($finding1 loss1$): Neg(Dot(Mul(Y,Add(1,Z)),Log(Softmax(X))))



Q: In a subsection of section 3.1, “Effectiveness of the Search Space”, the authors mention that **they introduce IoU into the cross entropy and focal loss, and show that they outperform the conventional cross entropy and focal loss. They then said this verifies the effectiveness of the search space. I am not seeing how this is connected to the effectiveness of the search space.**

A: We consider that the effectiveness of the search space indicates that there exists some effective loss functions within the proposed search space. After introducing the IoU into the search space, we have no idea if this new search space contains well-performed loss functions. So we attempt to design a loss function by hand to validate the effectiveness of the search space.

Q: **The regression branch contains fewer primitive operators because of the simplicity of the regression task.**

A: We say "simplicity of the regression task" to deliver that the gain brought by regression branch loss is less than classification branch. Specifically, it can be validated in Table 6 that best-discovered classification loss obtains 0.3 mAP more than regression loss. In fact, the reduced search space for regression branch is a tradeoff between performance and efficiency. With the reduced search space, we obtain similar well-performed regression loss. 

We will further clarify this in the paper in order to avoid confusion.
